CUPID pre-CDR

CUPID is a proposed future tonne-scale bolometric neutrinoless double beta decay ($0\nu\beta\beta$) experiment to probe the Majorana nature of neutrinos and discover Lepton Number Violation in the so-called inverted hierarchy region of the neutrino mass. CUPID will be built on experience, expertise and lessons learned in CUORE, and will exploit the current CUORE infrastructure as much as possible. In order to achieve its ambitious science goals, CUPID aims to dramatically reduce the backgrounds in the region of interest introducing a high efficiently $\alpha$/$\beta$ discrimination techniques, also demonstrated by the CUPID-0 and CUPID-Mo experiments, and using a high transition energy double beta decay nucleus, $^{100}$Mo. This document describe the main concepts related with the design of the CUPID experiment and indicates the projected sensitivities and the global scientific goal of the experiment.

==> TeO/TeO.tex <==
\subsection{Enriched $^{130}$TeO$_2$ production}
The enrichment of Te in $^{130}$Te introduces several new challenges. First, our early experiments \cite{Artusa2017} demonstrate that the enriched detectors had excessive radioactive backgrounds of thorium and uranium. Second, our experience with the CUORE crystals showed that about 30 to 35$\%$ of the TeO$_2$ input material ends up in the usable crystal. Third, crystals grown by SICCAS (Shanghai Institute of Ceramics of the Chinese Academy of Science), with the Bridgman technique, with seed crystals of natural abundance TeO$_2$, showed significant dilution of the enriched abundance.

Accordingly, the input Te or TeO$_2$ must be purified to reduce the Th and U content; the valuable scrap TeO$_2$ must be efficiently recycled, and the crystals must be either grown by the Czochralski method, where the seed crystals have negligible mass, or grown by the Bridgeman technique with enriched seed crystals grown by the Czochalski method.

To achieve the purification of the input material, we propose an experimental  effort to develop a technique to zone-refine TeO$_2$. If successful, this could also be used to recycle the scrap material from the crystal fabrication. Our team has explored chemical purification with the help of the Brookhaven National Laboratory, and we conclude that it is cost prohibitive. We discovered that SICCAS no longer grows crystals using the Czochralski method; however, Gooch and Housego Inc., in Cleveland Ohio routinly grows TeO$_2$ with the Czochralski technique.  

To explore the purification by zone-refinement, the University of South Carolina purchased a 1250 $^\circ$C, computer-controlled zone-furnace from MELLEN, Inc., in Concord, NH, with NSF funds previously awarded to explore the enrichment of CUORE. At the time of this writing, the zone refining facility is nearing completion, and funds are available to complete the installation, including the platinum zone boats, and natural abundance TeO$_2$ for the trials, and for some evaluation of the results by Inductively Coupled Plasma Mass Spectroscopy (ICPMS). The ICPMS tests are being explored in cooperation with the Pacific Northwest National Laboratory. The main funding required, and which is not on hand, is for additional enriched isotope to produce eight TeO$_2$ bolometers needed for an adequate test tower.

The CUPID project also involves an R$\&$D effort to explore the possibility to use bolometers grown from LiMoO$_4$, (lithium molybdate). It turns out that this compound melts at 703 $^\circ$C, compared to the melting temperature of TeO$_2$, which is 732 $^\circ$C. Both compounds require zone refinement boats made of platinum. Accordingly, the R$\&$D to explore the purification of input and scrap TeO$_2$ might also serve the LiMoO$_4$ option for CUPID.

We have identified one possible scenario to optimize the efficiency in the purification of the input TeO$_2$, as well as the recycling of the scrap material from the crystal fabrication. This option would have the TeO$_2$ crystals grown by the Czochralski method in the U.S. where zone-refinement would be used for both primary and recycling purification as shown in Fig.~\ref{fig:PurificationTeO}.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{TeO/figs/sec8_fig1.png}
    \caption{Potential scheme for purification of input material and recycling scrap TeO$_2$ from crystal fabrication.}
    \label{fig:PurificationTeO}
\end{figure}

We have been working with Gooch and Housego inc., (Cleveland, Ohio) to determine if producing the enriched TeO$_2$ CUORE crystals by the Czochralski technique would be cost competitive. This technique has a tiny seed and will not dilute the 130Te abundance. One advantage of growing the crystals in the US would be to avoid the expense and complications of shipping scrap back to the US, and returning reprocessed material back to China. Our experience with CUORE demonstrated that about 30$\%$ of the input material ended up in crystals. This implies that about 1.75 kg of oxide must be re-processed for each crystal pulled. If the crystals were produced a SICCAS, the many shipments of scrap material for reprocessing, and its return to SICCAS would be very complicated, costly and time consuming. In addition, SICCAS does not grow crystals by the Czochralski method, so large seed crystal seeds would have to be grown in the US and shipped to China periodically. In any case, a strong case can be made to develop the zone refining technique for TeO$_2$ and to attempt the similar technique for LiMoO$_4$.

==> infrastructure/assembly.tex <==
\subsection{Detector Assembly, Mounting, and Wiring}
In this subsection we describe the assembly procedure and facilities used for CUORE. At this stage of the conceptual design we expect many of these procedures will be similar for CUPID. We highlight lessons learned and areas which will differ and will need technical R\&D to develop procedures.  The assembly process for CUORE consisted of four steps: (i) gluing, i.e., fixing sensors the the TeO$_2$ crystals, (ii) mechanical assembly of the copper frames, crystals and Cu-PEN readout strips into towers, (iii) wirebonding, i.e., forming the electrical connection between sensors and the readout strips, and (iv) tower closing, extraction and storage.  The CUORE tower was composed by 13 identical floors, each composed by 4 bolometers, held in position by a composite structure and formed by pure copper frames (providing the necessary mechanical support) and PTFE holders (in order to get the most clean contact achievable to avoid crystals recontamination).  %{\color{red} FIXME describe some where the conceptual design for the CUPID towers}

\subsubsection{Environment, Space and Support Facilities}
The four main steps of assembly took place in the CUORE cleanrooms on the first floor of the CUORE hut underground at LNGS.  Gluing was performed in a dedication cleanroom (CR2) and proceeded independently of other activities in the hut. Mechanical assembly and wirebonding took place in CR3 and CR4 and took place through the so-called C-TAL (CUORE Towers Assembly Line). Exploiting a common interface represented by the so-called Universal Working Plane (UWP) and an extremely safe and controlled parking volume (so-called Garage), n.4 Glove Box were alternated - each one presenting specific features able to accomplish the requirements of each construction step -  in order to assembly and wire the several components in a clean environment, preserving the radio-purity of the detector under construction. An ancillary glove box was also used to prepare the sub-assemblies (so called End of the World Box) for the operations in the main ones, constituting - at the end - an overall 5-glove box system. However, this led to coupling of the mechanical assembly and wire-bonding which complicated scheduling activities. As noted below, wire-bonding for CUPID will need to be rethought and this is an opportunity decouple these tasks.  The heavy mechanical (and sometimes dirty) work of constructing the cryostat took place in CR5. This work often lead to vibrations which interfered with the delicate task of wire bonding. In reality CR5 could not be maintained as a clean room until the end of the cryostat commissioning. CR5 personal used the same entrance to the hut as personnel doing critically clean work in CR2,3 and 4. This lead to difficulties maintaining cleanliness of the cleanroom areas.   Completely decoupling CR5 from the other rooms would be desirable should heavy/dirty work be needed for cryostat upgrades for CUPID. 

As well as the underground cleanroom space in the CUORE hut, the core assembly tasks were supported by other facilities at LNGS.  Cleanrooms, wet benches and laminar flow hoods in the above ground chemical labs supported cleaning and processing of small parts such as heaters, thermistors, PTFE supports, and CuPEN readout strips and periodic cleaning of tools for assembly.  Lab space was provided for electrical testing of CuPEN strips. The underground parts storage area, adjacent to the CUORE hut was used to store parts prior to assembly as well as to store glued crystals prior to integration into towers.  A fume hood and cleanroom supported cleaning and reprocessing of thermistors and heaters for gluing attempts that did not pass our quality checks. 
We expect CUPID will require similar support.  %{\color{red} FIXME I did not mention here the various offsite production and QA facilities i.e heaters, NTDs, frames machining etc}

\subsubsection{Gluing}

As noted earlier, gluing was performed in CR2. The entire operation was carried out in a nitrogen-flushed glovebox to prevent recontamination of the crystals with radon. The system consisted of a station for crystal loading and inspection, which was carried out by a pair of human operators. A robotic arm moved crystals from the inspection station to a staging position in the glovebox. Precision so-called z-positioners were designed to hold the sensors (thermistors and heaters) in a fixed position relative to the crystal during gluing. The sensors were mounted on the positioner by a human operator while a second operator prepared glue for the upcoming operation. Once ready, a matrix of glue dots was precisely printed on the sensor by a second robotic arm. Inspection of the deposited glue matrix was done by a human operator with the aid of high resolution cameras and imaging processing software. If the glue matrix passed quality inspection the robotic arm moved a crystal from the staging area to the z-positioner allowing the crystal face to come into contact with the glue matrix. The glue was allowed to cure for 50 minutes. After curing, the glued crystal was repositioned to the staging area by the robotic arm. At the end of the operation the cured glue matrix was inspected by an operator with the aid of high-resolution cameras. The entire procedure was \emph{semi automatic} controlled by a GUI interface and operated by a team of three technicians and one physicist supervisor. A picture of the CUORE gluing tool is displayed in Fig.~\ref{fig:gluing}.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{infrastructure/figs/Gluing.jpg}
    \caption{Front view of the CUORE semi-automatic gluing tool. The robotic arm for crystal handling, the crystal and sensor staging, the two Z-positioners (hosting a crystal each) and the robotic arm for the glue deposition can be observed.}
    \label{fig:gluing}
\end{figure}

For CUPID additional sensor positioners will be needed because of the cylindrical geometry of LMO crystals and Ge wafer light detectors. In particular, the design of the latter can be made starting from the solution adopted during the gluing of the CUPID-0 detector. In this case the Ge wafer was encapsulated in a dedicated PTFE holder, allowing to handle them as "normal" crystals \cite{Azzolini:2018tum}.
The robotic positioning arm and glue dispensing arm will need to be reprogrammed to account for the different geometries and glue matrix patterns for each sensor-detector combination. In CUORE one tower worth of crystals were glued every two weeks, with operations mostly confined to a single 8-hour shift on weekdays. The time was dominated by the cure time of the glue, i.e., the time that had to elapse before moving on the next crystal The system had approximately 20\% downtime for routine and non-routine maintenance. Assuming a similar protocol for CUPID, doubling the number of detectors, i.e, main bolometer and light detector, we anticipate 96 weeks or two years to perform the gluing. We anticipate technical upgrades of the gluing system will take 1.5 years.%{\color{red}WAG}. 

\subsubsection{Mechanical Assembly}

Mechanical assembly of the glued crystals and copper frames into towers took place in CR3 and CR4. All steps were performed in specially designed task-specific nitrogen-flushed gloveboxes~\cite{Buccheri:2014bma}, the above mentioned C-TAL.  The operations include: (i) unpacking and quality checking of all copper and PTFE pieces, running-in of all threaded components to avoid gauling during the assembly; (ii) assembly of copper frames, PTFE holders and crystal into towers; (iii) gluing the left and right pack of CuPEN strips to their respective backing copper frame and allowing the glue to cure; (iv) attaching the CuPEN strip assemblies to the tower.  These operations involved n.3 different glove boxes: one for the mechanical assembly (Meck Box, see Fig.~\ref{fig:MechBox}), one for the preparation of the wirings on related cable trays (End Of the World Box, see Fig.~\ref{fig:eow}), and one for the installation of the cable trays on the tower (Cabling Box).  The main workstation was mounted on a stainless steel air-tight nitrogen flushed chamber equipped with an automated system able to lift and rotate the tower under-construction, as needed.  After the tower was assembled it was removed and stored in a nitrogen-flushed PMMA chamber, named the Storage Box of C-TAL (one per each tower), and parked inside dedicated racks equipped with nitrogen lines. This phase was performed by a team of 4 technicians working one eight-hour shift per day and it took one week to complete one tower.  Towers were typically assembled in batches of three and then the wirebonding team took over the workstation. We anticipate a similar pace of assembly can be achieved for {\cupid} but as discussed below the assembly sequence may need to be altered to accomodate wirebonding for the {\cupid} geometry.

\begin{figure}
\begin{minipage}[b][][t]{.5\linewidth}
\centering
\includegraphics[width=\linewidth]{infrastructure/figs/assembly01.jpg}
\caption{A CUORE tower under construction into the Mech Box.}
\label{fig:MechBox}
\end{minipage}
\begin{minipage}[b][][t]{.5\linewidth}
\centering
\includegraphics[width=\linewidth]{infrastructure/figs/EOW.jpg}
\caption{People working at the End Of the World Glove Box.}
\label{fig:eow}
\end{minipage}
\end{figure}


\subsubsection{Wirebonding} 
In CUORE, the tower design was such that all bonding pads on the sensors and CuPEN strips were accessible from the side of the tower after mechanical assembly. This allowed wirebonds connecting the sensor pads to the readout to be formed at any time. The wirebonder was modified to work in a horizontal mode rather that the typical vertical mode and was mounted on travelling rails to increase the range of motion. This, combined with the fine motion provided by automation of Garage, allowed for course positioning of the bonding head relative to the target pad. The final fine-positioning was achieved in the standard way using the integrated manipulator of the bonding machine. The entire setup was enclosed in a nitrogen flushed glovebox to avoid radon contamination of the tower - the so-called Bonding Box as well part of C-TAL system (see Fig.~\ref{fig:bonding}).  Each sensor was instrumented with four $\sim$ one-cm-long wires for a total of 416 wires per tower. The operation was performed by a team of two operators, one expert operating the wirebonder, the second controlled the course positioning of the tower and bonding machine.  Wirebonding was typically done in 12-hour shifts and it took about one week to bond a single tower.  Assembled towers were typically bonded in batches of three.  Once a tower was bonded it was returned to storage and the next tower to be bonded was placed on the Universal Working Plane (UWP).   

At this stage of the conceptual design, is unlikely that the same bonding protocol can be followed for {\cupid} and technical R\&D on a new protocol needs to proceed. The LMO crystals will have a cylindrical geometry and the curved outer surface will be wrapped in light reflecting foil. This constrains the sensors to be attached on one of the flat faces of the crystal. Thus sensors will not be accessible for bonding once assembled into a tower. Similar considerations apply to the Ge wafer light detectors which will be interposed between adjacent floors of the tower. A possible approach is to build stand-alone 4-crystal floors or modules and 4-wafer floors that can be stacked together into a tower. Each module could be instrumented with a set of readout strips that connect bonding pads near the sensor location to bonding pads that can be accessed from the side of the tower. The sensors could be bonded after assembly of the module and bonded modules could be stacked into towers later. Once the floors are stacked into towers the externally accessible pads could be wirebonded to the final readout. This would allow most of the wirebonding to proceed in parallel with gluing. Of course the tower assembly protocol would need to include measures to protect delicate wirebonds on each module during assembly.
This approach of having stand alone modules of pre-assembled LDs was successfully used for the construction of the towers of the CUPID-0 detector. In particular, thanks to dedicated 3D printed holding tools (see Fig.~\ref{fig:preAssembledLD}), it was possible to avoid the introduction of additional copper support frame to complete the light detector modules, thus having adjacent floors sharing a single frame as for the CUORE towers \cite{Azzolini:2018tum}.
\begin{figure}
\begin{minipage}[b][][t]{.5\linewidth}
\centering
\includegraphics[width=\linewidth]{infrastructure/figs/Bonding.jpg}
\caption{Bonding of a CUORE tower.}
\label{fig:bonding}
\end{minipage}
\begin{minipage}[b][][t]{.5\linewidth}
\centering
\includegraphics[width=\linewidth]{infrastructure/figs/assemblyLDCupid0.jpg}
\caption{A CUPID-0 LD pre-assembled in its 3D printed housing.}
\label{fig:preAssembledLD}
\end{minipage}
\end{figure}

\subsubsection{Closing and storage} 
The final step of CUORE assembly after wirebonding was to place protective copper covers over the CuPEN strip assemblies (using again the Cabling Box of C-TAL, see Fig.~\ref{fig:cabling}). These covers held to strip assemblies tightly against the frame so that they could not freely vibrate. The completed towers were then removed from the workstation and stored in individual nitrogen flushed boxes in CR4 (see Fig.~\ref{fig:storage}).  We anticipate similar storage arrangement will be adequate for CUPID. 

\begin{figure}
\begin{minipage}[b][][t]{.5\linewidth}
\centering
\includegraphics[width=\linewidth]{infrastructure/figs/Cabling.jpg}
\caption{People working with the Cabling Box}
\label{fig:cabling}
\end{minipage}
\begin{minipage}[b][][t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{infrastructure/figs/storage.jpg}
\caption{Some of the CUORE towers inside their storage box.}
\label{fig:storage}
\end{minipage}
\end{figure}

\subsubsection{Detector Installation}
The detectors hang from a so-called tower support plate which is in thermal contact with the 10~mK stage of the CUORE cryostat. A specially designed cart which provided for fine adjust the XYZ position and tilt of the tower was used to position the tower under the assigned spot beneath the tower support plate and raise it into position (Fig.~\ref{fig:install}, left).  The tower was then fixed to the support plate and the readout strips connected. The operations were carried out in a specially designed soft-walled cleanroom (CR6) which was supplied with radon free air.  The towers were installed by a team of three people at a rate of one per day.  For redundancy, a cylindrical plastic barrier (radon exclusion bag) could be quickly positioned around the bottom of the cryostat, covering the mounted towers. The exclusion bag was put in place and continuously flushed with nitrogen when personnel were not working in CR6 and when personnel entered or exited the room.  The pace of installation was set by the time needed for the radon level in CR6 to reduce to acceptable levels after entering or exiting the area, the time needed to re-clean the working area and tools before the next operation, and the desire not to overexert the operators performing the critical and stressful installation task.  We anticipate a similar setup and protocol will be adequate for {\cupid}.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{infrastructure/figs/towers_installed.png}
    \caption{Installation of the CUORE towers. The top part of the plastic radon exclusion bag is visible around the tower support plate. Left: an operator positions a tower using the cart. Right: tower installation completed.}
    \label{fig:install}
\end{figure}

==> infrastructure/clean_rooms.tex <==
%Tommy and Carlo
\subsection{Cleanrooms}
\label{sec:cleanroom}
A cleanroom environment will be needed for assembly and storage of the CUPID detectors. We plan to reuse the cleanroom facilities developed for CUORE. The first floor of the CUORE hut houses a class 1000 cleanroom with approximately 100 m$^2$ floor space.  The cleanroom is divided into five sub volumes which we call CR1,CR2,CR3,CR4 and CR5.  CR1 is an entrance area 
\begin{figure}
\begin{minipage}[b][][t]{.6\linewidth}
\centering
\includegraphics[width=\linewidth]{infrastructure/figs/CUORE-hut-1.pdf}
\caption{Rendering of the CUORE hut underground at LNGS. The cleanroom facilities are located on the first floor.}
\label{fig:screws}
\end{minipage}
\begin{minipage}[b][][t]{.3\linewidth}
\centering
\includegraphics[width=\linewidth]{infrastructure/figs/cleanrooms-map2.pdf}
\caption{Floor map of CUORE cleanrooms}
\label{fig:cleanrooms}
\end{minipage}

\end{figure}

==> lightdetectors/lightdetector.tex <==
\section{Light detectors} 
%\emph{Coordinator: M. Vignati}

Based on the experience gained in the framework of the CUPID R$\&$D projects, we selected Ge-based light detectors with NTD-Ge readout for CUPID. As detailed in the next section, the features and the performances of the Light Detectors (LD) which employ this technique satisfy the requirements for CUPID, with the advantage of exploiting the same electronics and the wiring system already implemented in CUORE. Several R\&Ds are still underway to develop more sensitive and faster LDs: NTD with Neganov-Luke amplification, Transition Edge Sensors (TES) and Kinetic Inductance Detectors (KIDs). To complement the light detectors, R\&Ds on the optimization of the light collection and of the mechanical supports are carried out.
 
\subsection{Baseline technology: Ge light absorbers with NTD sensors}
\label{sec:Ge_LD_NTD}

Ge-based light detectors instrumented with NTD-Ge temperature sensors are one of the most well-established technologies for scintillation light detection in cryogenic experiments \cite{Bellini:2018,Pirro:2017,Poda:2017c}. The NTD readout of the light detectors is also important to take advantage of the electronics and the wiring system already implemented in the CUORE experiment. The long-standing experience acquired in the framework of the bolometric double-beta  experiments LUCIFER \cite{Beeman:2013b}, which is now running as CUPID-0 \cite{Artusa:2016,Azzolini:2018tum}, LUMINEU \cite{Armengaud:2017,Poda:2017d} and its extension CUPID-Mo \cite{Poda:2018} allows to reach robust very high performances in terms of energy resolution, stability and reliability. The performances of the light detectors developed by the CUPID-0, LUMINEU and CUPID-Mo collaborations are summarized in Table~\ref{tab:LDGeNTD_performances}. The recent CUPID R\&D results on development of a fast Ge-based optical bolometer \cite{Barucci:2019ghi} are also listed in Table~\ref{tab:LDGeNTD_performances} and illustrated in Fig.~\ref{fig:LD_NTD_calibration}.


\begin{table}
\centering
\caption{
\todo{FB: Do we want to clean up the table leaving only the most relevant information? DP: On my mind the info here is very useful taking into account that it concerns the baseline option}
Performances (harmonic mean) of NTD-Ge instrumented light detectors based on Ge slabs with the size of $\oslash 44.5 \times 0.175$~mm. Table quotes the results achieved in the CUPID-0 (currently running), LUMINEU (completed) and CUPID-Mo (recently started) experiments. Also the recent results achieved in the framework of the CUPID R\&D program are quoted.}
%\normalsize
\footnotesize
%\scriptsize
%\tiny 
\begin{center}
\begin{tabular}{l|cc|c|cc|c}
\hline\noalign{\smallskip}
~ & \multicolumn{2}{|c|}{{\bf CUPID-0}} 		& {\bf LUMINEU} & \multicolumn{2}{|c|}{{\bf CUPID-Mo}}  & {\bf CUPID R\&D}	\\
~  & \cite{Artusa:2016} 	& \cite{Azzolini:2018tum} & \cite{Poda:2017d}	& commissioning 	& upgraded 	&\cite{Barucci:2019ghi} \\
\hline
SiO coating  				& \multicolumn{2}{|c|}{Single side}											& Single side								& \multicolumn{2}{|c|}{Double side}  &None\\
NTD Ge size (mm) 			& \multicolumn{2}{|c|}{2.8$\times$2.0$\times$0.5}				&	2.2$\times$0.8$\times$0.6 & 3.0$\times$0.8$\times$0.4 & 2.8$\times$0.8$\times$1.1 &2.85$\times$1$\times$0.4 \\
Operated detectors   		& 6													& 31 												&	4$^a$							& 17$^b$		& 17$^c$									& 1 \\
Time of test (yr)    		& 0.1												& 2  												&	0.3												& 0.2												& 0.3		& 0.1										 \\				
\hline
Temperature (mK)   			& 20.0											& 17.5											&	17.0											& 20.5											& 20.0		& 15 									 \\
NTD R$_{work}$ (M$\Omega$) 	& 0.8										& 4.2 											&	0.7												& 1.2												& 0.8				&   1.5								 \\	
\hline
Rise time (ms)      		& 1.8												& 3.5 											&	2.0												& 0.8												& 1.2					& 0.8							 \\				
Decay time (ms) 				& 5													& 7													& 13												& 6													&	13	&1.6											 \\				
\hline
Signal ($\mu$V/keV) 		& 1.3												& --$^d$										&	1.5$^e$										& 1.2												& 0.96							&3.9					 \\				
Baseline RMS (eV) 			& 41 												& --$^d$										&	35$^e$										& 167$^f$										& 58								    & 20			 \\	
\hline
\multicolumn{7}{l}{$^a$ --- One similar performance detector was with a 2.2$\times$1.3$\times$0.6 mm NTD.} \\ 
\multicolumn{7}{l}{$^b$ --- Two of them were with 2.2$\times$0.8$\times$0.6-mm and 2.2$\times$0.8$\times$0.3 mm NTDs.} \\ 
\multicolumn{7}{l}{$^c$ --- A half of similar performance detectors operate with slightly different NTDs: five of them are 3.0$\times$0.8$\times$1.0 mm} \\ 
\multicolumn{7}{l}{sensors, two thermistors are 2.2$\times$0.8$\times$0.6 mm NTDs and one has a size of 3.0$\times$0.8$\times$0.4 mm.} \\ 
\multicolumn{7}{l}{$^d$ --- No light detector calibration has been available yet.} \\ 				\multicolumn{7}{l}{$^e$ --- Limited by the necessity to operate at low R$_{work}$ values because of the AC bias electronics \cite{Armengaud:2017}. Improved} \\ 
\multicolumn{7}{l}{performance were obtained in measurements at 17 mK with the DC-polarized CUORE-like electronics at CSNSM:} \\
\multicolumn{7}{l}{3.4 $\mu$V/keV signal and 28 eV baseline noise RMS (NTD R$_{work}$ = 4.5 M$\Omega$).} \\
\multicolumn{7}{l}{$^f$ --- Affected by an extra 1/f noise due to the lack of cut NTDs polishing (see text).} \\ 	
\end{tabular}
 \label{tab:LDGeNTD_performances}
\end{center}

\end{table} 



\begin{figure*}[htbp]
\begin{center}
\resizebox{\textwidth}{!}{\includegraphics{lightdetectors/figs//GeNTDnew.pdf}}
\end{center}
\caption{Performance of a Ge-LD tested at LNGS in the framework of the CUPID R$\&$D program~\cite{Barucci:2019ghi}. {\it Left.} Energy distribution of the random sampled noise. The width of the distribution ($\sigma$ = 20 eV) represents the baseline energy resolution of the Ge-LD. In the right inset the $^{55}$Fe calibration spectrum of the Ge-LD. The x-axis unit is in absolute voltage drop across the thermistor. The RMS resolution on the 5.9 keV and 6.5 keV X-ray peaks is 59 eV. {\it Right.} Rise and decay times distributions corresponding to the $^{55}$Fe X-rays. The Bessel cut-off frequency of the Front-End is 550 Hz.}
 \label{fig:LD_NTD_fastGe}
\end{figure*} 


For the abovementioned reasons, the baseline design for the CUPID light detectors is a disk-shaped pure Ge bolometer, with a double side SiO anti-reflecting coating, instrumented with NTD-Ge thermistors. Ge substrates, provided by UMICORE Electro-Optic Material (Geel, Belgium), are double side polished wafers of diameter 50 mm and an average thickness of 175 $\mu$m, with an impurity concentration below 2~$\times$~10$^{10}$ atoms/cm$^3$. Prior the light detectors construction, each wafer will be coated on both sides by a 70~nm SiO anti-reflecting layer \cite{Mancuso:2014,Azzolini:2018tum}, which enhances the light collection by a factor of two \cite{Artusa:2016}. A small NTD-Ge sensor (with a mass of 15 mg or less) will be glued on the Ge surface using the same gluing tools as the main Li$_2$MoO$_4$ crystals. To avoid an issue of a large 1/f extra noise issue in cut NTDs (faced over the CUPID-Mo commissioning), it is strongly necessary to perform a dedicated polishing of thermistors (done in the CUPID-0). It is worth mentioning that the use of $\sim$1 mg NTD Ge sensors would allow to get a faster response, to further increase the signal amplitude and to reduce the baseline noise \cite{Coron:2004,Armengaud:2017} (see also in Table~\ref{tab:LDGeNTD_performances}). The Ge wafer will be held by PTFE clamps in a copper housing. The thermal link to the heat sink is provided by $\oslash$25-$\mu$m Au bonding wires which give also the electrical connection with the NTD Ge sensors. 



\subsection{Neganov-Luke assisted NTD}\label{sec:NL-NTD}

Standard NTD equipped, Ge or Si-absorber-based light detectors can be upgraded to exploit the so-called Neganov-Luke amplification mechanism \cite{Luke:1988} by adding a set of electrodes on the absorber surface(s)(NL-NTD, Fig. \ref{fig:NL-NTD}), in order to apply a static electric field to the semiconductor. The realization relies on well-assessed evaporation, sputtering and ion implantation techniques.
\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.3]{lightdetectors/figs//NL-NTD.jpg}
    \caption{Picture of a NL-NTD base germanium light detector. The absorber is realized with a $\oslash$=44~mm, 175~$\mu m$ thickness high purity germanium wafer. Concentric annular electrodes are deposited on the surface, which is then coated with a thin SiO (blue-ish) layer to enhance the photon absorption in the visible wavelength.}
    \label{fig:NL-NTD}
\end{figure}
\begin{figure}[h!]
\centering
\includegraphics[scale=0.3]{lightdetectors/figs//NL-NTD_Si.jpg}
\caption{Picture of a NL-NTD base silicon light detector. The absorber is realized with a 50$\times$50 mm, 625~$\mu m$ high-resistivity silicon. Electrodes of different geometries can be realized by ion implantation to realize ohmic contacts.}
\label{fig:NL-NTD_Si}
\end{figure}
By this amplification mechanism typical performances reached are of 10 $\sim $20~uV/keV responsivity and 10 $\sim$ 20~eV (FWHM) baseline resolution under grid bias up to 70~V (300~V), corresponding to a factor $\sim$10 (50) improvement in the signal-to-noise ratio with respect to the standard Ge (Si) detectors. Several NL-NTD prototypes of about 15~cm$^2$ (up to 25~cm$^2$ with Si) detection surface have been realized 
and operated several time in above-ground experiments and in underground facilities (LNGS, LSM) to perform R\&D measurements where a specific low energy detection was required, well beyond the limit one could get with standard NTD equipped light detectors. 
\todo{(Here or in the TeO chapter? It seems confusing to me switching between TeO and LMO in this section)}. 
In particular a TeO$_2$ CUORE composite bolometer, equipped with a NL-NTD to exploit the Cherenkov light, could reach an $\alpha$ rejection factor of 99.9\% with a $\gamma(\beta)$ acceptance level of about 96\% \cite{PRC_TeO2}.

The technique of the NL-NTD light detectors is now-a-day mature to be deployed in a large scale experiment, allowing to reach detection thresholds of about 10 times smaller than the standard NTD light detector, with a minimal price to pay of 2(1) additional wires(detector), required to bias the electrode sets.

\subsection{Transition Edge Sensors}
\input{lightdetectors/TES/tes}\label{sec:TES}

\subsection{Kinetic Inductance Detectors}\label{sec:MKID}
Kinetic Inductance Detectors (KIDs) have been successfully applied in astro-physics searches providing superb energy resolution and natural multiplexed read-out~\cite{Day:2013}. Because the active surface of these devices is limited to few mm$^2$ they can be operated as cryogenic light detector in $0\nu\beta\beta$ search only exploiting the phonon-mediated approach, proposed by Swenson et al.~\cite{Swenson:2010yf} and Moore et al.~\cite{Moore:2012au}.

\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.35]{lightdetectors/KID/figs/figurePoissonCalGaussians.pdf}
    \includegraphics[scale=0.35]{KID/figurePoissonCal.pdf}
    \caption{Left: Histograms of pulse heights in the phase readout for light signals of different energies. Right: Standard deviation $\sigma$ versus mean m of the Gaussian distributions shown in the left panel. The plot includes one more point at 65 mrad not shown in the left panel to not compress the scale for the other distributions. The curve is well described by the Poisson statistics of photons. The resolution at zero amplitude corresponds to 25~eV~RMS. See Ref.~\cite{Cardani:2018krv} for more details.}
    \label{fig:KIDResult}
\end{figure}
In such an approach, KIDs are deposited on a large insulating substrate featuring a surface of several cm$^2$. Then, scintillation or Cherenkov photons emitted by cryogenic calorimeters interact with the substrate producing phonons which travel within until a small fraction of them (5-10~\%) are absorbed by a KID.
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.3]{lightdetectors/KID/figs/KIDPulse.pdf}
    \caption{Phase (Red) and amplitude (blue) variation measured from the center of the resonance loop induced by optical pulses produced with a 400~nm LED lamp located at room temperature and routed inside the cryostat by an optical fiber. The photon burst had a time duration of 1~$\mu$s.}
    \label{fig:KIDpulse}
\end{figure}
Exploiting the phonon-mediated technique, the CALDER project~\cite{Battistelli:2015vha}, realized a cryogenic light detector using a $2\times2$~cm$^2$ Si substrate 300~$\mu$m thick monitored with one aluminum KID. The detector showed a baseline energy resolution of about 80~eV~RMS, constant in a temperature range starting from 10~mK up to 200~mK~\cite{Bellini:2016lgg}. Moving from Al to more sensitive superconductors, such as AlTiAl multi-layer, the baseline energy resolution has improved up to 25~eV~RMS~\cite{Cardani:2018krv}. The high energy resolution of this prototype allowed to obtain a solid estimation of the detector performance exploiting an absolute energy calibration based on the Poisson statistics of the photons absorbed into the substrate as shown in Fig.~\ref{fig:KIDResult}.
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.35]{lightdetectors/KID/figs/Elba_Si_NOISE.pdf}
    \includegraphics[scale=0.35]{lightdetectors/KID/figs/Elba_SOS_NOISE.pdf}
    \caption{Noise power spectra measured for the same Al resonator evaporated on Si (left) and silicon on sapphire, i.e. SOS, (right) substrates with pulse tube off (red line) and on (black line). The noise increase at low frequency caused by the vibrations induced by the pulse tube is visible only for Si substrates.}
    \label{fig:KIDNoise}
\end{figure}
A very important feature of KIDs is their fast time response as shown in Fig~\ref{fig:KIDpulse}. The typical rise and decay time, indeed, are $10^2$ times faster than NTD Ge thermistors increasing substantially the capability to reject pile-up events. This would allow to further suppress the background coming from the $2\nu\beta\beta$ pile-up events in $^{100}$Mo enriched cryogenic calorimeters. 
\todo{(further suppress if needed? otherwise it seems our baseline is not satisfactory)}. 
Furthermore, exploiting sapphire substrates instead of silicon, KIDs result barely affected by the mechanical vibrations induced by pulse tube refrigerator. This is shown in Fig.~\ref{fig:KIDNoise} where an increase of the detector noise at low frequency is visible when the pulse tube is operating only for Si substrates. Despite this effect was observed in all the sapphire substrates measured, a clear explanation of this experimental evidence has not been yet formulated.
In summary, in addition to offering a sensitivity competitive with the NTDs, KIDs provide a stronger reduction of the background events coming from pile-up thanks to the faster time response and overcome the problems caused by the mechanical vibrations induced by pulse tube refrigerators that, in NTD and TES based detectors could lead to a worsening of the baseline energy resolution.


\input{lightdetectors/LightCollectionOptimization}

\subsection{Thermal and Mechanical Support}
The baseline-energy resolutions achieved by massive low temperature calorimeters are a few of orders of magnitude worse than theoretical predictions. It has been pointed out by Matt Pyle et al., \cite{Pyle:2015arxiv} that this effect can occur when there is a mismatch between the signal and sensor bandwidths. If the coupling between the photon absorber and the thermal bath is larger than the thermal coupling between the absorber and the sensor, this can lead to sub-optimal collection of signal phonons in the sensor. This in turn leads to degradation of the energy resolution.

An ideal weak link should have an extremely low heat capacity and thermal conductance.  While polytetrafluoroethene (PTFE) has been extensively and reliably used over the last decade as the weak thermal link between the absorber and the thermal bath, it does add a non-negligible parasitic heat capacity to the device, affecting its performance. We are currently working towards developing suitable alternatives that can offer better bandwidth matching for next generation detectors. A single crystal sapphire (Al$_2$O$_3$) seems to be the most ideal due to its extremely low heat capacity.  One can also utilize the thermal boundary resistance between sapphire and copper (thermal bath) to further reduce the thermal coupling between the absorber and thermal bath. On the other hand, increasing the thermal coupling between sensor and the absorber using suitable number of gold wire bonds can also help tune the signal bandwidth. 

However, unlike PTFE, sapphire is not easily machinable. We are looking at the feasibility of using sapphire as a support structure for the light detectors. Further testing to optimize the mounting arrangement and device characterization is underway.

